Low-Rank Koopman Deformables with Log-Linear Time Integration

We present a low-rank Koopman operator formulation for accelerating deformable subspace simulation. Using a Dynamic Mode Decomposition (DMD) parameterization of the Koopman operator, our method learns the temporal evolution of deformable dynamics and predicts future states through efficient matrix evaluations instead of sequential time integration. This yields log-linear scaling in the number of time steps and allows large portions of the trajectory to be skipped while retaining accuracy. The resulting temporal efficiency is especially advantageous for optimization tasks such as control and initial-state estimation, where the objective often depends largely on the final configuration. To broaden the scope of Koopman-based reduced-order models in graphics, we introduce a discretization-agnostic extension that learns shared dynamic behavior across multiple shapes and mesh resolutions. Prior DMD-based approaches have been restricted to a single shape and discretization, which limits their usefulness for tasks involving geometry variation. Our formulation generalizes across both shape and discretization, which enables fast shape optimization that was previously impractical for DMD models. This expanded capability highlights the potential of Koopman operator learning as a practical tool for efficient deformable simulation and design.

==> sections/method.tex <==
\section{Discontinuity Modeling via Restricting Higher-Dimensional Continuous Functions}
\label{sec:method}
Our core idea is to constrain a higher-dimensional continuous function (neural field) $B$ onto a height field $H(\mathbf{x})$ that encodes the discontinuities. This height field captures the discontinuities by satisfying the condition
\[
\lim_{\mathbf{x} \to \partial\Omega^{+}} H(\mathbf{x}) \neq \lim_{\mathbf{x} \to \partial\Omega^{-}} H(\mathbf{x}).
\]
Instead of using just the spatial coordinate $\mathbf{x}$ as input, we lift the input dimension by combining the spatial coordinate with the height field value, resulting in the pair $\left( H(\mathbf{x}), \mathbf{x} \right)$. This lifting ensures that points from both sides, ${\mathbf{x}_1 \to \partial\Omega^{+}}$ and ${\mathbf{x}_2 \to \partial\Omega^{-}}$, are mapped to distinct higher-dimensional positions within the neural field $B$, as shown in \reffig \ref{fig:IllusLifting}. During inference of the continuous function $B$, the two points, which are very close in the rest state (${\mathbf{x}_1 \to \partial\Omega^{+}}$ and ${\mathbf{x}_2 \to \partial\Omega^{-}}$), are mapped sufficiently far apart in the higher dimension $\left( H(\mathbf{x}), \mathbf{x} \right)$ because $H$ lifts them to different heights in the additional dimension.

\begin{figure}
\centering
\includegraphics[width=2cm]{example-image-duck}
\caption{
Lifting the input of the continuous function.
} 
\label{fig:IllusLifting} 
\centering
\end{figure}

The benefit of lifting is that it decouples spatial discontinuity from the trainable continuous function $B$. Without lifting, the function $B$ must be very unsmooth at the boundary $\partial \Omega$ to accommodate the discontinuity, which complicates training. However, our method alleviates this problem. By lifting, two positions $ \mathbf{x}_1 \to \partial \Omega^{+} $ and $ \mathbf{x}_2 \to \partial \Omega^{-} $, which are close in $ \Omega $, are mapped to distinct coordinates in a higher dimension. This allows $B$ to remain smooth everywhere, with the discontinuity arising from restricting the function to the discontinuous height field. As a result, training the function becomes easier, as no sharp jumps need to be fit, as shown in \reffig \ref{fig:WhyEasier}. 


\begin{figure}
\centering
\includegraphics[width=2cm]{example-image-duck}
\caption{
The trainable function $B$ is smooth over the higher dimensional domain, making the training process easier. (also show lower MSE in this figure)
} 
\label{fig:WhyEasier} 
\centering
\end{figure}


This height field isn't subject to strict constraints. Any function that satisfies 
$  \lim_{\mathbf{x} \to \partial \Omega^{+}} H(\mathbf{x}) \neq \lim_{\mathbf{x} \to \partial \Omega^{-}} H(\mathbf{x}) $
can be used. We use the generalized winding number to construct the height field, as it has been proven to satisfy this property \cite{Feng:2023:WND, Jacobson:2018:GWN, Barill:FW:2018} and is computationally efficient.






%Since the generalized winding number field naturally captures the jumping boundary condition at the boundaries, the points from both sides of the discontinuities are lifted to different higher dimensional positions within the higher-dimensional nerual field. Therefore, we 
